Scalable Approximation Algorithm for Network Immunization

The problem of identifying important players in a given network is of pivotal importance for viral marketing, public health management, network security and various other fields of social network analysis. In this work we find the most important vertices in a graph G = (V,E) to immunize so as the chances of an epidemic outbreak is minimized. This problem is directly relevant to minimizing the impact of a contagion spread (e.g. flu virus, computer virus and rumor) in a graph (e.g. social network, computer network) with a limited budget (e.g. the number of available vaccines, antivirus software, filters). It is well known that this problem is computationally intractable (it is NP-hard). In this work we reformulate the problem as a budgeted combinational optimization problem and use techniques from spectral graph theory to design an efficient greedy algorithm to find a subset of vertices to be immunized. We show that our algorithm takes less time compared to the state of the art algorithm. Thus our algorithm is scalable to networks of much larger sizes than best known solutions proposed earlier. We also give analytical bounds on the quality of our algorithm. Furthermore, we evaluate the efficacy of our algorithm on a number of real world networks and demonstrate that the empirical performance of algorithm supplements the theoretical bounds we present, both in terms of approximation guarantees and computational efficiency.

==> Notation.tex <==
\section*{Notation}
\begin{itemize}
	\item For a graph $G$, $A(G)$ denotes the adjacency matrix of $G$ or just $A$ when graph in context is clear.
	\item For a subset of vertices $S$, $G_S$ is the subgraph induced by vertices in $S$ and $A_S$ represents its adjacency matrix.
	\item For $S\in V$, $G^{[S]}=G_{V\setminus S}$, that is it denotes the subgraph obtained after removing the vertices of $S$. And $A^{[S]}$ is its adjacency matrix.
	\item For a set $X\subset V(G)$, and vertex $v\in V(G)$, $N_X(v)=N_{G_X}(v)$ is the set of neighbors of $v$ in $X$ and $d_X(v)=d_{G_X}(v)=|N_X(v)|$, called degree of $v$ in $X$. When $X=V(G)$, we refer to $d_G(v)$ as $d(v)$.
	\item Let $u,v \in V(G)$ and $X\subset V(G)$, $d_X(u,v)$ represents the size of common neighborhood of $u$ and $v$ in set $X$, i.e $d_X(u,v)=|N_X(u)\cap N_X(v)|$
	\item $\{\lambda_i(G)\}_{i=1}^n$ or $\{\lambda_i(A)\}_{i=1}^n$ is the eigen spectrum of graph $G$ or matrix $A$.
	\item $\lambda_{max}(G)=\max_{i} \lambda_i(G)$
	
	
\end{itemize}
For a set $X\subset V(G)$, and vertices $u,v\in V(G)$, $N_X(v)=N_{G_X}(v)$ is the set of neighbors of $v$ in $X$ and $d_X(v)=d_{G_X}(v)=|N_X(v)|$, called degree of $v$ in $X$. When $X=V(G)$, we refer to $d_G(v)$ as $d(v)$. Moreover $d_X(u,v)$ represents the size of common neighborhood of $u$ and $v$ in set $X$, i.e $d_X(u,v)=|N_X(u)\cap N_X(v)|$. For a vertex $v\in S\subset V(G)$, $\cCW_p(v,S)$ is the set of all closed walks of length $p$ in $G_S$ containing $v$ at least once and $cw_p(v,S)=|\cCW_p(v,S)|$. Similarly we define $\cCW_p(S,G)$ to be the set of closed walks of length $p$ containing vertices of $S$ and correspondingly $cw_p(S,G)$ is the cardinality of the set. For simplicity we write $cw_p(G,G)$ as $cw_p(G)$.
